Predicting Fault-Ride-Through Probability of Inverter-Dominated Power Grids using Machine Learning

Due to the increasing share of renewables, the analysis of the dynamical behavior of power grids gains importance. Effective risk assessments necessitate the analysis of large number of fault scenarios. The computational costs inherent in dynamic simulations impose constraints on the number of configurations that can be analyzed. Machine Learning (ML) has proven to efficiently predict complex power grid properties. Hence, we analyze the potential of ML for predicting dynamic stability of future power grids with large shares of inverters. For this purpose, we generate a new dataset consisting of synthetic power grid models and perform dynamical simulations. As targets for the ML training, we calculate the fault-ride-through probability, which we define as the probability of staying within a ride-through curve after a fault at a bus has been cleared. Importantly, we demonstrate that ML models accurately predict the fault-ride-through probability of synthetic power grids. Finally, we also show that the ML models generalize to an IEEE-96 Test System, which emphasizes the potential of deploying ML methods to study probabilistic stability of power grids.

==> removed_text.tex <==

% The main contributions are:
% \begin{itemize}
%     \item Generation of a dataset of synthetic power grid models with appropriate models for inverters and loads and the computation of their fault-ride-through probability ($p_{frt}$).
%     \item Successful application of different ML concepts to predict $p_{frt}$ of synthetic power grid models.
%     \item Evaluation of the capability of ML to generalize to different power grids, such as the on a IEEE96 Test system, which is not used for training.
% \end{itemize}
% - ML method can predict $p_{frt}$
% - GNNs achieve better performance than non-graph ML methods
% - ML can also generalize to a differently structured IEEE test case
% - To conduct the training of ML methods, we generated a new dataset of inverter-based power grids
% - As required by ENTSOE, we showed the feasability of conducting probabilistic stability assessment of the dynamical behavior power grid models. 
% - The generated datasets highlight the relevance of topological structures, which serves as an indicator for the strong performance of GNNs.

% - The study shows the potential of ML to predict probabilistic stability of future power grids
    % The generated more realistic datasets are a further step on the path to real-world applications. GNNs are able to predict the dynamic stability of power grid models and outperform baselines that purely rely on nodal features as input. Thus highlighting the importance of including topological properties into the ML approach. As a strong challenge, out-of-distribution generalization is tested by predicting the dynamic stability of an IEEE test case and observe good performances of all ML models. Following earlier studies that analyzed more simplified power grid models, the great performances on the more challenging datasets underline the potential of the approach. The results show that ML methods can be beneficial when analyzing future power grids where dynamical effects are of great importance. Due to the fast evaluation times, there are almost no limits for the number of configurations that can be analyzed. This can help to improve the quality of power grid operating by enabling the automatic analysis of numerous configurations and potentially for power grid planing by considering dynamic effects at early stages.

%% abstract

% Abstract—Due to the increasing share of renewables, the analysis
% of the dynamical behavior of power grids gains importance.
% Effective risk assessments necessitate the analysis of large number
% of fault scenarios. The computational costs inherent in dynamic
% simulations impose constraints on the number of configurations
% that can be analyses. Machine Learning (ML) has proven to effi-
% ciently predict complex power grid properties. Hence, we analyze
% their potential for predicting dynamic stability of future power
% grids with large shares of inverters. We generate new datasets
% comprising synthetic power grid models, perform dynamical
% simulations to calculate the fault-ride-through probability pf rt.
% We employ these datasets for training Machine Learning (ML)
% models. Importantly, we demonstrate that ML accurately predict
% FRTP of synthetic power grids and also generalize to an IEEE-96
% Test System, emphasizing the potential of ML methods to study
% different power grid configurations.


        % Since the IEEE test case provides us only with 72 data points, the comparison may be vulnerable to small changes. Hence, the performances differences on the IEEE test case should not be emphasized too much, but the general feasibility of predicting the dynamic stability of the IEEE case can be observed, even though its properties are quite different from the synthetic power grids. 
        
% can play a major role to reduce the computational effort by predicting complex patterns. In comparison to the literature, where ML predicts the dynamic stability of coupled oscillator networks, more realistic synthetic datasets are generated and the performance of multiple ML models is compared. The power grid models mimic features of future power grids with large shares of grid-forming inverters. It can be demonstrated that ML can be used to predict the dynamic stability. GNNs significantly outperform ML-methods that only consider the nodal features, underlining the importance of topological properties. To show the potential for future applications, the generalization to an IEEE-96 Test System, that is not used for training, but validation purposes only, is demonstrated. The trained models generalize to this unknown new structure, emphasizing the potential of ML methods to study different power grid configurations.
    
    %, which serve as simplified representations of power grid models. 
    
    % Lastly, GNNs are also used for probabilistic stability assessment of simplified power grid models \cite{nauckPredictingBasinStability2022,nauckDynamicStabilityAnalysis2022,nauckDynamicStabilityAssessment2023}. However, in the latter publications, a paradigmatic model for power grids was chosen, using fixed line admittances and less sophisticated bus modeling. Both, generators and loads have been modeled with the swing equation. Furthermore, the authors only considered asymptotic stability and did not consider operational bounds. In this paper, more realistic power grids are generated and GNNs are tested on a more advanced challenge.



% removed literature
% short-term photovoltaic (PV) power forecasting \cite{zhangOptimalGraphStructure2023}

% phasor measurement- based event identification \cite{yuanLearningLatentInteractions2023}
% There are many applications of ML-methods in the context of power grids \cite{xieReviewMachineLearning2020,kumbharComprehensiveReviewMachine2021} and depending on the task different strategies appear to work best. In case of important topological properties or when analyzing changing topologies, Graph Neural Networks (GNNs) are particularly appropriate. GNNs can deal with full graphs as inputs, whereas other, more conventional methods require some kind of preprocessing to properly provide the inputs to ML. For example, instead of using the full graphs as input, several methods consider nodal features only. The authors of \cite{liaoReviewGraphNeural2022} provide an overview of different applications. In general, there is a strong focus on power-flow related tasks, such as \cite{beinertPowerFlowForecasts2023}. There is also prediction of transients \cite{nandanooriGraphNeuralNetwork2022,sunFastTransientStability2022}, as well as probabilistic stability assessment of simplified power grid models \cite{nauckPredictingBasinStability2022,nauckDynamicStabilityAnalysis2022,nauckDynamicStabilityAssessment2023}. However, in the latter publications, power grids are rudimentary modeled as oscillator networks, using fixed line admittances and less sophisticated bus modeling. Both, generators and loads are modeled with the swing equation. Furthermore, the authors only considered asymptotic stability and did not consider operational bounds. As a next step, more realistic power grids are generated and GNNs are tested on a more sophisticated challenge.
% \paragraph{Our main contributions are}



        % \subsection{Scaling input data}
        % We investigate the influence of using no scaling, standardization and min-max-normalization. The following setup is used for the min-max-normalization:
        % \begin{align}
        %     x' = a + \frac{(x-\min(x))(b-a)}{\max(x)-\min(x)}, \\
        % \end{align}
        % where $a,b$ are chosen in dependence on the $\min(x)$ and $\max(x)$:
        % \begin{align}
        %     a, b =
        %     \begin{cases}
        %         -1, 1, \quad \text{if} \quad \min(x) < 0 \quad \& \quad \max(x) > 0 \\
        %         1, 0, \quad \text{if} \quad \min(x) <= 0 \quad \& \quad \max(x) <= 0 \\
        %         0, 1 \quad \text{if} \quad \min(x) >= 0 \quad \& \quad \max(x) >= 0 \\
        %     \end{cases}
        % \end{align}


        % Lately, there are many more GNN layers of increasing complexity introduced and especially Graph Attention Networks \cite{velickovicGraphAttentionNetworks2018,brodyHowAttentiveAre2022} achieve good overall performance. They make use of computing attentions to contribute for different importance of the considered buses, details can be found in \cite{velickovicGraphAttentionNetworks2018,brodyHowAttentiveAre2022}. 

% \section{Prediction of SURV using ML}
% In case of GNNs, we use three different approaches to deal with the input data. First, we differ between a homogeneous and a heterogeneous setup. In case of the homogeneous setup, all buses get the same 6 nodal input features. For the heterogeneous setup, the loads and normal form buses are treated differently, considering the additional input features for the normal form buses. That means that different graph convolutions are used for the different possible combinations of bus connections. To account for the different number of input features, the dimension of the first convolutional layer. We only apply the heterogeneous setup in case of GAT. The TAG, we further simplify the input by only providing nodal features as input. However, some of the line features are still considered, they are incorporated in the sum of the corresponding line features for each bus.





% \begin{table*}[h]
%     \centering
%     \caption{This tables gives an overview on the used input features for the training of the ML models.}
%     \begin{tabularx}{\linewidth}{p{2cm}p{1.5cm}XXp{2.5cm}}
%          model & setup & nodal features & line features & number of parameters\\
%          regression & homo & P,Q, $\mathcal{R} (B_x)$, $G_k$, $B_k$, $B_{k,sh}$ & $G_{km}$, $B_{km}$, $B_{km, sh}$, $P_{km}$, $Q_{km}$& 6\\
%          GBT & homo & P,Q, & & -\\
%          TAG & homo & P,Q, & \\
%          GAT & homo & P,Q, & \\
%          GAT & hetero & P,Q, & \\
%     \end{tabularx}
%     \label{tab:model_inputs}
% \end{table*}



% \begin{table}[h]
%     \centering
%     \caption{The results of predicting survivability using $R^2$ in \% with different ML applications.-reg denotes model with stronger regularization.}
%     \begin{tabularx}{\linewidth}{XXXX}
%          model & setup & test set & ieee case \\
%          regression & homo & 62.10 & 72.02 \\
%          GBT & homo & 62.88 & 72.39 \\
%          TAG & homo &  & \\
%          GAT & homo &  & \\
%          GAT& hetero &  & \\
%          \hline
%          GAT-regul & homo &  & \\
%          GAT-regul & hetero &  & \\
%          TAGrel & homo &  & \\
%     \end{tabularx}
%     \label{tab:results_old}
% \end{table}
\end{document}


The details of the final models are provided in \Cref{tb_model_properties}.

\begin{table}[!t]
	\centering
	\caption{Properties of models. Number of parameters denotes the number of learnable weights of the model.}
    \begin{tabularx}{\linewidth}{p{2cm}XX}
		\toprule
		name &  number of layers & number of parameters \\
		\midrule
		TAGNet  & 3 &  \\
	   \bottomrule
 	\end{tabularx}
	\label{tb_model_properties}
\end{table}

